QUIJOTE scientific results -- V. The microwave intensity and polarisation spectra of the Galactic regions W49, W51 and IC443

We present new intensity and polarisation maps obtained with the QUIJOTE experiment towards the Galactic regions W49, W51 and IC443, covering the frequency range from 10 to 20 GHz at $\sim$ 1 deg angular resolution, with a sensitivity in the range 35-79 ${\mu}$K/beam for total intensity and 13-23 ${\mu}$K/beam for polarisation. For each region, we combine QUIJOTE maps with ancillary data at frequencies ranging from 0.4 to 3000 GHz, reconstruct the spectral energy distribution and model it with a combination of known foregrounds. We detect anomalous microwave emission (AME) in total intensity towards W49 at 4.7${\sigma}$ and W51 at 4.0${\sigma}$ with peak frequencies ${\nu}_{AME}$ = (20.0 $\pm$ 1.4) GHz and ${\nu}_{AME}$ = (17.7 $\pm$ 3.6) GHz respectively; this is the first detection of AME towards W51. The contamination from ultra-compact HII regions to the residual AME flux density is estimated at 10% in W49 and 5% in W51, and does not rule out the AME detection. The polarised SEDs reveal a synchrotron contribution with spectral indices ${\alpha}_s$ = -0.67 $\pm$ 0.10 in W49 and ${\alpha}_s$ = -0.51 $\pm$ 0.07 in W51, ascribed to the diffuse Galactic emission and to the local supernova remnant respectively. Towards IC443 in total intensity we measure a broken power-law synchrotron spectrum with cut-off frequency ${\nu}_{0,s}$ = (114 $\pm$ 73) GHz, in agreement with previous studies; our analysis, however, rules out any AME contribution which had been previously claimed towards IC443. No evidence of polarised AME emission is detected in this study.

==> tables/depol_table.tex <==
\begin{table*}
\centering
\caption{For both W49 and W51, and for both the case of the original resolution and the smoothed \textit{Planck}-HFI map at 353 GHz, we report the integrated $I$, $Q$ and $U$ fluxes inside the chosen apertures. We then quote the polarisation fluxes and polarisation fractions computed in two different ways. $P^{\rm (aps)}$ is computed from the $Q$, and $U$ flux densities, yielding the polarisation fraction $\Pi^{\rm (aps)}$. $P^{\rm (aps)}$ is computed integrating the polarisation values for individual pixels in the aperture, yielding the polarisation fraction $\Pi^{\rm (aps)}$.}
\label{tab:depolarisation}
\setlength{\tabcolsep}{1.em}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{ccccccccccc}
\hline
\hline
\\[-1em]
\multicolumn{11}{c}{W49} \\ 
\\[-1em]
\hline
\\[-1em]
 Reso. & $r_{\rm ap}$  & $I$ &  $Q$ & $U$ & & $P^{\rm (aps)}$ &  $\Pi^{\rm (aps)}$ & & $P^{\rm (pix)}$ &  $\Pi^{\rm (pix)}$ \\ 
\\[-1em]
 ['] & ['] & [Jy] & [Jy] & [Jy] & & [Jy] & [\%] & & [Jy] & [\%]  \\ 
\\[-1em]
\hline
\\[-1em]
\\[-1em]
5 & 19 & 2326.0 & 12.2 & 19.8 &  & 23.3 & 1.0 &  & 22.8 & 1.0\\
\\[-1em]
\\[-1em]
60 & 60 & 9666.2 & 190.2 & 43.9 &  & 195.2 & 2.0 &  & 181.1 & 1.9\\
\\[-1em]
\hline
\hline
\\[-1em]
\multicolumn{11}{c}{W51} \\ 
\\[-1em]
\hline
\\[-1em]
 Reso. & $r_{\rm ap}$  & $I$ &  $Q$ & $U$ & & $P^{\rm (aps)}$ &  $\Pi^{\rm (aps)}$ & & $P^{\rm (pix)}$ &  $\Pi^{\rm (pix)}$ \\ 
\\[-1em]
 ['] & ['] & [Jy] & [Jy] & [Jy] & & [Jy] & [\%] & & [Jy] & [\%]  \\ 
\\[-1em]
\hline
\\[-1em]
\\[-1em]
5 & 30 & 5300.1 & -19.9 & 60.1 &  & 63.3 & 1.2 &  & 58.1 & 1.1\\
\\[-1em]
\\[-1em]
60 & 80 & (1.6) $\times 10^{4}$ & 159.5 & 93.0 &  & 184.6 & 1.1 &  & 175.9 & 1.1\\
\\[-1em]
\hline
\hline
\end{tabular}
\end{table*}


==> tables/w49_errtable.tex <==
\begin{table*}
\centering
\caption{Comparison between older (1) and newer (2) versions of the error estimates in $I$, $Q$ and $U$ for W49 together with their percent variations.}
\label{tab:w49_errs}
\setlength{\tabcolsep}{1em}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{cc|ccc|ccc|ccc}
\hline
\hline
\multicolumn{11}{c}{W49}\\
\hline
Survey & Freq. & $\sigma_{I}^{(1)}$ & $\sigma_{I}^{(2)}$ & $\Delta\sigma_{I}$ & $\sigma_{Q}^{(1)}$ & $\sigma_{Q}^{(2)}$ & $\Delta\sigma_{Q}$ & $\sigma_{U}^{(1)}$ & $\sigma_{U}^{(2)}$ & $\Delta\sigma_{U}$\\
 & [GHz] & [Jy] & [Jy] & [\%] & [Jy] & [Jy] & [\%] & [Jy] & [Jy] & [\%]\\
\hline
\hline
Haslam & 0.4 & 28.4 & 94.5 & 233 &  -  &  -  &  -  &  -  &  -  &  - \\
Berkhuijsen & 0.8 & 16.9 & 58.1 & 245 &  -  &  -  &  -  &  -  &  -  &  - \\
Reich & 1.4 & 10.2 & 57.1 & 459 &  -  &  -  &  -  &  -  &  -  &  - \\
DRAO & 1.4 &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  - \\
Jonas & 2.3 & 8.9 & 52.1 & 486 & 2.1 & 2.4 &  17 & 1.2 & 1.0 &  19\\
Urumqi & 4.8 & 7.8 & 54.7 & 600 & 7.8 & 54.7 & 600 & 7.8 & 54.7 & 600\\
QUIJOTE & 11.1 & 4.3 & 37.1 & 761 & 0.6 & 0.7 &  15 & 0.5 & 0.4 &  21\\
QUIJOTE & 12.9 & 4.5 & 39.2 & 780 & 0.6 & 0.7 &  11 & 0.3 & 0.3 &  23\\
QUIJOTE & 16.8 & 5.0 & 44.6 & 785 & 0.3 & 0.6 &  92 & 0.2 & 0.2 &   5\\
QUIJOTE & 18.8 & 5.3 & 45.7 & 766 & 0.3 & 0.5 &  73 & 0.2 & 0.2 &   8\\
\textit{WMAP} & 22.8 & 4.7 & 45.7 & 868 & 0.3 & 0.5 &  66 & 0.2 & 0.3 &  51\\
\textit{Planck}-LFI & 28.4 & 4.3 & 41.9 & 871 & 0.2 & 0.3 &  94 & 0.2 & 0.2 &  33\\
\textit{WMAP} & 33.0 & 3.7 & 45.0 & 1103 & 0.3 & 0.4 &  27 & 0.2 & 0.3 &  26\\
\textit{WMAP} & 40.6 & 2.9 & 42.5 & 1381 & 0.4 & 0.3 &  22 & 0.3 & 0.3 &   1\\
\textit{Planck}-LFI & 44.1 & 3.7 & 34.5 & 835 & 0.2 & 0.3 &  59 & 0.2 & 0.2 &   6\\
\textit{WMAP} & 60.8 & 3.3 & 43.1 & 1225 & 0.4 & 0.9 & 106 & 0.6 & 0.5 &  28\\
\textit{Planck}-LFI & 70.4 & 5.0 & 37.6 & 656 & 0.3 & 0.3 &   3 & 0.3 & 0.2 &  21\\
\textit{WMAP} & 93.5 & 7.6 & 73.0 & 866 & 2.0 & 2.5 &  26 & 1.6 & 2.8 &  70\\
\textit{Planck}-HFI & 100.0 & 9.0 & 70.1 & 678 & 0.5 & 1.1 & 109 & 0.3 & 0.6 & 111\\
\textit{Planck}-HFI & 143.0 & 19.9 & 173.7 & 772 & 1.5 & 3.1 & 107 & 0.9 & 1.5 &  67\\
\textit{Planck}-HFI & 217.0 & 91.0 & 764.5 & 741 & 6.4 & 14.3 & 125 & 4.2 & 7.5 &  78\\
\textit{Planck}-HFI & 353.0 & 495.1 & 3605.2 & 628 &  -  &  -  &  -  &  -  &  -  &  - \\
\textit{Planck}-HFI & 545.0 & 1735.6 & 13230.4 & 662 &  -  &  -  &  -  &  -  &  -  &  - \\
\textit{Planck}-HFI & 857.0 & 5679.4 & 44349.0 & 681 &  -  &  -  &  -  &  -  &  -  &  - \\
DIRBE & 1249.1 & 5638.7 & 138578.7 & 2358 &  -  &  -  &  -  &  -  &  -  &  - \\
DIRBE & 2141.4 & 8741.2 & 205709.0 & 2253 &  -  &  -  &  -  &  -  &  -  &  - \\
DIRBE & 2997.9 & 3330.8 & 95838.2 & 2777 &  -  &  -  &  -  &  -  &  -  &  - \\
\hline
\hline
\end{tabular}
\end{table*}


==> tables/w51_errtable.tex <==
\begin{table*}
\centering
\caption{Comparison between older (1) and newer (2) versions of the error estimates in $I$, $Q$ and $U$ for W51 together with their percent variations.}
\label{tab:w51_errs}
\setlength{\tabcolsep}{1em}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{cc|ccc|ccc|ccc}
\hline
\hline
\multicolumn{11}{c}{W51}\\
\hline
Survey & Freq. & $\sigma_{I}^{(1)}$ & $\sigma_{I}^{(2)}$ & $\Delta\sigma_{I}$ & $\sigma_{Q}^{(1)}$ & $\sigma_{Q}^{(2)}$ & $\Delta\sigma_{Q}$ & $\sigma_{U}^{(1)}$ & $\sigma_{U}^{(2)}$ & $\Delta\sigma_{U}$\\
 & [GHz] & [Jy] & [Jy] & [\%] & [Jy] & [Jy] & [\%] & [Jy] & [Jy] & [\%]\\
\hline
\hline
Haslam & 0.4 & 47.4 & 132.7 & 180 &  -  &  -  &  -  &  -  &  -  &  - \\
Berkhuijsen & 0.8 & 29.0 & 98.2 & 239 &  -  &  -  &  -  &  -  &  -  &  - \\
Reich & 1.4 & 15.6 & 62.3 & 299 &  -  &  -  &  -  &  -  &  -  &  - \\
DRAO & 1.4 &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  -  &  - \\
Jonas & 2.3 & 15.9 & 67.0 & 321 & 2.1 & 3.4 &  60 & 1.8 & 1.2 &  35\\
Urumqi & 4.8 & 8.4 & 76.1 & 808 & 8.4 & 76.1 & 808 & 8.4 & 76.1 & 808\\
QUIJOTE & 11.1 & 5.3 & 53.7 & 906 & 0.7 & 0.4 &  51 & 0.7 & 0.7 &   2\\
QUIJOTE & 12.9 & 6.0 & 55.5 & 826 & 0.5 & 0.7 &  39 & 0.8 & 0.7 &   6\\
QUIJOTE & 16.8 & 5.9 & 61.3 & 932 & 0.3 & 0.6 &  66 & 0.5 & 0.4 &   6\\
QUIJOTE & 18.8 & 6.1 & 63.4 & 937 & 0.5 & 0.9 &  83 & 0.4 & 0.5 &  41\\
\textit{WMAP} & 22.8 & 5.6 & 63.6 & 1035 & 0.2 & 0.6 & 183 & 0.4 & 0.4 &   1\\
\textit{Planck}-LFI & 28.4 & 4.4 & 57.7 & 1216 & 0.3 & 0.4 &  39 & 0.3 & 0.2 &  39\\
\textit{WMAP} & 33.0 & 4.8 & 64.3 & 1233 & 0.4 & 0.6 &  64 & 0.4 & 0.3 &  11\\
\textit{WMAP} & 40.6 & 4.6 & 61.4 & 1230 & 0.5 & 0.4 &  13 & 0.4 & 0.4 &   8\\
\textit{Planck}-LFI & 44.1 & 4.0 & 49.4 & 1122 & 0.2 & 0.5 & 121 & 0.3 & 0.3 &   4\\
\textit{WMAP} & 60.8 & 8.4 & 65.4 & 681 & 0.9 & 0.6 &  35 & 0.5 & 1.0 & 109\\
\textit{Planck}-LFI & 70.4 & 7.4 & 56.5 & 661 & 0.6 & 0.7 &  21 & 0.5 & 0.3 &  38\\
\textit{WMAP} & 93.5 & 18.3 & 112.0 & 511 & 3.0 & 2.5 &  16 & 1.9 & 2.6 &  35\\
\textit{Planck}-HFI & 100.0 & 14.3 & 106.8 & 646 & 0.7 & 1.1 &  51 & 0.4 & 0.7 &  69\\
\textit{Planck}-HFI & 143.0 & 32.7 & 257.7 & 689 & 2.2 & 3.5 &  58 & 1.3 & 1.8 &  40\\
\textit{Planck}-HFI & 217.0 & 166.0 & 1078.8 & 550 & 9.1 & 16.1 &  77 & 4.7 & 5.4 &  17\\
\textit{Planck}-HFI & 353.0 & 847.8 & 5057.3 & 497 &  -  &  -  &  -  &  -  &  -  &  - \\
\textit{Planck}-HFI & 545.0 & 2978.9 & 18531.2 & 522 &  -  &  -  &  -  &  -  &  -  &  - \\
\textit{Planck}-HFI & 857.0 & 9247.4 & 61010.7 & 560 &  -  &  -  &  -  &  -  &  -  &  - \\
DIRBE & 1249.1 & 15067.6 & 175286.5 & 1063 &  -  &  -  &  -  &  -  &  -  &  - \\
DIRBE & 2141.4 & 22730.3 & 263443.2 & 1059 &  -  &  -  &  -  &  -  &  -  &  - \\
DIRBE & 2997.9 & 12086.8 & 117801.9 & 875 &  -  &  -  &  -  &  -  &  -  &  - \\
\hline
\hline
\end{tabular}
\end{table*}

